Hyperspectral CNN Classification with Limited Training Samples

Hyperspectral imaging sensors are becoming increasingly popular in robotics applications such as agriculture and mining, and allow per-pixel thematic classification of materials in a scene based on their unique spectral signatures. Recently, convolutional neural networks have shown remarkable performance for classification tasks, but require substantial amounts of labelled training data. This data must sufficiently cover the variability expected to be encountered in the environment. For hyperspectral data, one of the main variations encountered outdoors is due to incident illumination, which can change in spectral shape and intensity depending on the scene geometry. For example, regions occluded from the sun have a lower intensity and their incident irradiance skewed towards shorter wavelengths. In this work, a data augmentation strategy based on relighting is used during training of a hyperspectral convolutional neural network. It allows training to occur in the outdoor environment given only a small labelled region, which does not need to sufficiently represent the geometric variability of the entire scene. This is important for applications where obtaining large amounts of training data is labourious, hazardous or difficult, such as labelling pixels within shadows. Radiometric normalisation approaches for pre-processing the hyperspectral data are analysed and it is shown that methods based on the raw pixel data are sufficient to be used as input for the classifier. This removes the need for external hardware such as calibration boards, which can restrict the application of hyperspectral sensors in robotics applications. Experiments to evaluate the classification system are carried out on two datasets captured from a field-based platform.

==> conclusion.tex <==
%\section{conclusion}
%This work has proposed a method for training a CNN to be robust to several factors of variation in hyperspectral data with only a limited amount of training data. This was done through relighting augmentation using an approximation of the irradiance ratio found from the scene.  This work also showed that it is possible to train a CNN to classify hyperspectral data without first radiometrically normalising it using a calibration panel in the scene, which is a common practice for machine learning algorithms trained on spectral data. This has paved the way for utilisation of CNN's with hyperspectral cameras in robotics and other autonomous applications.
%
%Future work involves the incorporation of spatial information such that the filters are convolving both spectrally and spatially. Also, work will be done to increase the number of classes that a CNN can classify, similar to the very large classifiers trained on RGB image databases.
